Heterogeneous Treatment and Spillover Effects under Clustered Network Interference

The bulk of causal inference studies rule out the presence of interference between units. However, in many real-world scenarios, units are interconnected by social, physical, or virtual ties, and the effect of the treatment can spill from one unit to other connected individuals in the network. In this paper, we develop a machine learning method that uses tree-based algorithms and a Horvitz-Thompson estimator to assess the heterogeneity of treatment and spillover effects with respect to individual, neighborhood, and network characteristics in the context of clustered networks and neighborhood interference within clusters. The proposed Network Causal Tree (NCT) algorithm has several advantages. First, it allows the investigation of the treatment effect heterogeneity, avoiding potential bias due to the presence of interference. Second, understanding the heterogeneity of both treatment and spillover effects can guide policy-makers in scaling up interventions, designing targeting strategies, and increasing cost-effectiveness. We investigate the performance of our NCT method using a Monte Carlo simulation study, and we illustrate its application to assess the heterogeneous effects of information sessions on the uptake of a new weather insurance policy in rural China.

==> Tables/Old/correlated_025.tex <==
\begin{table}[H]
\scriptsize
\centering
\caption{Simulations' results for the first scenario with correlated covariates (0.25)}
\label{tab:correlated_0.25}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc}
\multicolumn{1}{l}{} & \multicolumn{7}{c}{\textit{Treatment Effects}}                                                                                    \\ \cline{2-8} 
\textit{Effect Size} & $\hat{\tau}_{l_1}$ & $\hat{se}(\hat{\tau}_{l_1})$ & $\hat{\tau}_{l_2}$ & $\hat{se}(\hat{\tau}_{l_2})$ & MSE   & Bias   & Coverage \\ \hline
0.1                  & 0.116              & 0.288                        & -0.230             & 0.225                        & 0.071 & -0.057 & 1.000    \\
1.1                  & 1.093              & 0.280                        & -1.078             & 0.288                        & 0.080 & 0.008  & 0.946    \\
2.1                  & 2.084              & 0.403                        & -2.067             & 0.401                        & 0.147 & 0.009  & 0.939    \\
3.1                  & 3.112              & 0.553                        & -3.134             & 0.555                        & 0.273 & -0.011 & 0.958    \\
4.1                  & 4.082              & 0.692                        & -4.140             & 0.699                        & 0.400 & -0.029 & 0.961    \\
5.1                  & 5.126              & 0.843                        & -5.162             & 0.852                        & 0.673 & -0.018 & 0.950    \\
6.1                  & 6.121              & 1.007                        & -6.157             & 1.008                        & 1.000 & -0.018 & 0.948    \\
7.1                  & 7.019              & 1.161                        & -7.067             & 1.165                        & 1.214 & -0.024 & 0.958    \\
8.1                  & 8.018              & 1.309                        & -8.085             & 1.309                        & 1.557 & -0.033 & 0.959    \\
9.1                  & 9.221              & 1.509                        & -9.088             & 1.491                        & 2.014 & 0.066  & 0.953    \\
10.1                 & 10.214             & 1.655                        & -10.195            & 1.648                        & 2.441 & 0.009  & 0.957    \\ \hline
                     & \multicolumn{7}{c}{\textit{Spillover Effects}}                                                                                    \\ \cline{2-8} 
                     & $\hat{\delta}_{l_1}$ & $\hat{se}(\hat{\delta}_{l_1})$ & $\hat{\delta}_{l_2}$ & $\hat{se}(\hat{\delta}_{l_1})$ & MSE   & Bias   & Coverage \\ \hline
0.1                  & 0.069              & 0.185                        & -0.200             & 0.194                        & 0.025 & -0.065 & 0.944    \\
1.1                  & 1.102              & 0.227                        & -1.090             & 0.227                        & 0.046 & 0.006  & 0.970    \\
2.1                  & 2.111              & 0.302                        & -2.117             & 0.302                        & 0.078 & -0.003 & 0.972    \\
3.1                  & 3.093              & 0.392                        & -3.116             & 0.393                        & 0.112 & -0.011 & 0.983    \\
4.1                  & 4.086              & 0.488                        & -4.093             & 0.490                        & 0.169 & -0.004 & 0.979    \\
5.1                  & 5.131              & 0.589                        & -5.078             & 0.587                        & 0.246 & 0.026  & 0.971    \\
6.1                  & 6.071              & 0.692                        & -6.051             & 0.693                        & 0.331 & 0.010  & 0.979    \\
7.1                  & 7.109              & 0.801                        & -7.087             & 0.802                        & 0.458 & 0.011  & 0.980    \\
8.1                  & 8.092              & 0.906                        & -8.063             & 0.902                        & 0.577 & 0.014  & 0.976    \\
9.1                  & 9.110              & 1.016                        & -9.060             & 1.010                        & 0.659 & 0.025  & 0.990    \\
10.1                 & 10.122             & 1.123                        & -10.101            & 1.124                        & 0.861 & 0.010  & 0.980    \\ \hline
\end{tabular}%
%}
\end{table}

==> Tables/Old/correlated_050.tex <==
\begin{table}[H]
\scriptsize
\centering
\caption{Simulations' results for the first scenario with correlated covariates (0.50)}
\label{tab:correlated_0.50}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc}
\multicolumn{1}{l}{} & \multicolumn{7}{c}{\textit{Treatment Effects}}                                                                                    \\ \cline{2-8} 
\textit{Effect Size} & $\hat{\tau}_{l_1}$ & $\hat{se}(\hat{\tau}_{l_1})$ & $\hat{\tau}_{l_2}$ & $\hat{se}(\hat{\tau}_{l_2})$ & MSE   & Bias   & Coverage \\ \hline
0.1                  & 0.129              & 0.223                        & -0.101             & 0.217                        & 0.050 & 0.014  & 0.909    \\
1.1                  & 1.093              & 0.268                        & -1.120             & 0.272                        & 0.066 & -0.014 & 0.972    \\
2.1                  & 2.140              & 0.392                        & -2.114             & 0.378                        & 0.158 & 0.013  & 0.949    \\
3.1                  & 3.104              & 0.503                        & -3.065             & 0.505                        & 0.241 & 0.019  & 0.946    \\
4.1                  & 4.123              & 0.652                        & -4.188             & 0.664                        & 0.399 & -0.033 & 0.960    \\
5.1                  & 5.081              & 0.795                        & -5.108             & 0.801                        & 0.618 & -0.013 & 0.953    \\
6.1                  & 6.138              & 0.960                        & -6.146             & 0.943                        & 0.825 & -0.004 & 0.959    \\
7.1                  & 7.154              & 1.110                        & -7.063             & 1.096                        & 1.088 & 0.045  & 0.956    \\
8.1                  & 8.093              & 1.227                        & -8.174             & 1.257                        & 1.388 & -0.041 & 0.949    \\
9.1                  & 9.080              & 1.380                        & -9.116             & 1.389                        & 1.637 & -0.018 & 0.959    \\
10.1                 & 10.086             & 1.529                        & -10.122            & 1.520                        & 1.952 & -0.018 & 0.952    \\ \hline
                     & \multicolumn{7}{c}{\textit{Spillover Effects}}                                                                                    \\ \cline{2-8} 
                     & $\hat{\delta}_{l_1}$ & $\hat{se}(\hat{\delta}_{l_1})$ & $\hat{\delta}_{l_2}$ & $\hat{se}(\hat{\delta}_{l_1})$ & MSE   & Bias   & Coverage \\ \hline
0.1                  & 0.144              & 0.190                        & -0.202             & 0.175                        & 0.030 & -0.029 & 0.864    \\
1.1                  & 1.091              & 0.214                        & -1.087             & 0.212                        & 0.047 & 0.002  & 0.952    \\
2.1                  & 2.103              & 0.282                        & -2.137             & 0.285                        & 0.064 & -0.017 & 0.975    \\
3.1                  & 3.119              & 0.364                        & -3.072             & 0.365                        & 0.097 & 0.024  & 0.977    \\
4.1                  & 4.098              & 0.458                        & -4.090             & 0.458                        & 0.156 & 0.004  & 0.962    \\
5.1                  & 5.056              & 0.551                        & -5.101             & 0.553                        & 0.218 & -0.022 & 0.976    \\
6.1                  & 6.127              & 0.654                        & -6.093             & 0.649                        & 0.302 & 0.017  & 0.980    \\
7.1                  & 7.093              & 0.750                        & -7.130             & 0.752                        & 0.370 & -0.018 & 0.988    \\
8.1                  & 8.162              & 0.852                        & -8.038             & 0.844                        & 0.476 & 0.062  & 0.984    \\
9.1                  & 9.122              & 0.948                        & -9.026             & 0.943                        & 0.571 & 0.048  & 0.982    \\
10.1                 & 10.043             & 1.046                        & -10.177            & 1.052                        & 0.698 & -0.067 & 0.982    \\ \hline
\end{tabular}%
%}
\end{table}

==> Tables/Old/homophily.tex <==
\begin{table}[H]
\scriptsize
\centering
\caption{Simulations' results for the first scenario with network homophily  within the clusters (30 clusters)}
\label{tab:homophily}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc}
\multicolumn{1}{l}{} & \multicolumn{7}{c}{\textit{Treatment Effects}}                                                                                    \\ \cline{2-8} 
\textit{Effect Size} & $\hat{\tau}_{l_1}$ & $\hat{se}(\hat{\tau}_{l_1})$ & $\hat{\tau}_{l_2}$ & $\hat{se}(\hat{\tau}_{l_2})$ & MSE   & Bias   & Coverage \\ \hline
0.1                  & 0.152              & 0.241                        & -0.108             & 0.259                        & 0.045 & 0.022  & 1.000    \\
1.1                  & 1.069              & 0.312                        & -1.094             & 0.315                        & 0.100 & -0.013 & 0.953    \\
2.1                  & 2.130              & 0.454                        & -2.119             & 0.448                        & 0.188 & 0.006  & 0.959    \\
3.1                  & 3.149              & 0.608                        & -3.083             & 0.606                        & 0.335 & 0.033  & 0.955    \\
4.1                  & 4.099              & 0.775                        & -4.084             & 0.763                        & 0.477 & 0.007  & 0.959    \\
5.1                  & 5.115              & 0.946                        & -5.116             & 0.943                        & 0.736 & 0.000  & 0.961    \\
6.1                  & 6.162              & 1.127                        & -6.150             & 1.127                        & 1.043 & 0.006  & 0.970    \\
7.1                  & 7.076              & 1.285                        & -7.175             & 1.289                        & 1.377 & -0.049 & 0.955    \\
8.1                  & 8.129              & 1.465                        & -8.000             & 1.446                        & 1.752 & 0.064  & 0.957    \\
9.1                  & 9.029              & 1.621                        & -9.136             & 1.629                        & 2.249 & -0.053 & 0.953    \\
10.1                 & 10.163             & 1.814                        & -10.133            & 1.815                        & 2.977 & 0.015  & 0.957    \\ \hline
                     & \multicolumn{7}{c}{\textit{Spillover Effects}}                                                                                    \\ \cline{2-8} 
                     & $\hat{\delta}_{l_1}$ & $\hat{se}(\hat{\delta}_{l_1})$ & $\hat{\delta}_{l_2}$ & $\hat{se}(\hat{\delta}_{l_1})$ & MSE   & Bias   & Coverage \\ \hline
0.1                  & 0.084              & 0.221                        & -0.142             & 0.222                        & 0.036 & -0.029 & 0.971    \\
1.1                  & 1.082              & 0.268                        & -1.100             & 0.274                        & 0.069 & -0.009 & 0.957    \\
2.1                  & 2.102              & 0.370                        & -2.084             & 0.366                        & 0.120 & 0.009  & 0.964    \\
3.1                  & 3.116              & 0.483                        & -3.112             & 0.486                        & 0.172 & 0.002  & 0.974    \\
4.1                  & 4.065              & 0.603                        & -4.114             & 0.610                        & 0.260 & -0.025 & 0.976    \\
5.1                  & 5.101              & 0.740                        & -5.077             & 0.737                        & 0.389 & 0.012  & 0.980    \\
6.1                  & 6.076              & 0.871                        & -6.045             & 0.869                        & 0.538 & 0.015  & 0.979    \\
7.1                  & 7.088              & 1.004                        & -7.054             & 0.997                        & 0.738 & 0.017  & 0.972    \\
8.1                  & 8.041              & 1.132                        & -8.150             & 1.142                        & 0.936 & -0.055 & 0.971    \\
9.1                  & 9.157              & 1.275                        & -9.030             & 1.263                        & 1.070 & 0.064  & 0.976    \\
10.1                 & 10.066             & 1.408                        & -10.093            & 1.407                        & 1.391 & -0.014 & 0.982    \\ \hline
\end{tabular}%
%}
\end{table}

==> Tables/Old/main_scenario1_10.tex <==

\vspace{2cm}
\begin{table}[H]
\scriptsize
\centering
\caption{Simulations' results for the first scenario (10 clusters)}
\label{tab:10clusters}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc}
\multicolumn{1}{l}{}                     & \multicolumn{7}{c}{\textit{Treatment Effects}}                                                                                                                                                                                                                                                                                  \\ \cline{2-8} 
\multicolumn{1}{l}{\textit{Effect Size}} & 
$\hat{\tau}_{\ell_1}$ &$\hat{se}(\hat{\tau}_{\ell_1})$ & 
$\hat{\tau}_{\ell_2}$ & $\hat{se}(\hat{\tau}_{\ell_2})$ & MSE                     & Bias                     & Coverage                     \\ \toprule
0.1                                      & 0.353                                           & 0.416                                                              & -0.139                                          & 0.350                                                              & 0.106                   & 0.107                    & 1.000                        \\
1.1                                      & 1.108                                           & 0.514                                                              & -1.132                                          & 0.515                                                              & 0.261                   & -0.012                   & 0.936                        \\
2.1                                      & 2.124                                           & 0.740                                                              & -2.156                                          & 0.741                                                              & 0.570                   & -0.016                   & 0.941                        \\
3.1                                      & 3.004                                           & 1.003                                                              & -3.050                                          & 0.997                                                              & 0.934                   & -0.023                   & 0.945                        \\
4.1                                      & 4.061                                           & 1.293                                                              & -4.179                                          & 1.287                                                              & 1.843                   & -0.059                   & 0.928                        \\
5.1                                      & 5.201                                           & 1.565                                                              & -5.197                                          & 1.585                                                              & 2.297                   & 0.002                    & 0.946                        \\
6.1                                      & 6.179                                           & 1.889                                                              & -6.086                                          & 1.824                                                              & 3.282                   & 0.046                    & 0.931                        \\
7.1                                      & 7.125                                           & 2.140                                                              & -7.110                                          & 2.128                                                              & 4.276                   & 0.007                    & 0.921                        \\
8.1                                      & 8.011                                           & 2.378                                                              & -8.149                                          & 2.425                                                              & 5.087                   & -0.069                   & 0.931                        \\
9.1                                      & 9.153                                           & 2.729                                                              & -9.128                                          & 2.713                                                              & 6.803                   & 0.012                    & 0.927                        \\
10.1                                     & 9.991                                           & 2.947                                                              & -9.916                                          & 2.974                                                              & 8.007                   & 0.038                    & 0.934                        \\ \midrule 
\multicolumn{1}{l}{}                     & \multicolumn{7}{c}{\textit{Spillover Effects}}                                                                                                                                                                                                                                                                                  \\ \cline{2-8} 
\multicolumn{1}{l}{}          & 
$\hat{\delta}_{\ell_1}$ & $\hat{se}(\hat{\delta}_{\ell_1})$ & 
$\hat{\delta}_{\ell_2}$ & $\hat{se}(\hat{\delta}_{\ell_2})$ & {MSE} & {Bias} & {Coverage} \\ \hline
0.1                                      & 0.225                                           & 0.380                                                              & -0.249                                          & 0.322                                                              & 0.082                  & -0.012                  & 0.958                       \\
1.1                                      & 1.114                                           & 0.415                                                              & -1.103                                          & 0.402                                                              & 0.155                  & 0.005                   & 0.960                       \\
2.1                                      & 2.085                                           & 0.542                                                              & -2.138                                          & 0.545                                                              & 0.230                  & -0.026                  & 0.967                       \\
3.1                                      & 3.047                                           & 0.716                                                              & -3.094                                          & 0.716                                                              & 0.408                  & -0.023                  & 0.972                       \\
4.1                                      & 4.098                                           & 0.892                                                              & -4.079                                          & 0.882                                                              & 0.646                  & 0.009                   & 0.966                       \\
5.1                                      & 5.119                                           & 1.063                                                              & -5.054                                          & 1.057                                                              & 0.862                  & 0.032                   & 0.958                       \\
6.1                                      & 6.090                                           & 1.250                                                              & -6.045                                          & 1.242                                                              & 1.132                  & 0.022                   & 0.958                       \\
7.1                                      & 7.086                                           & 1.437                                                              & -7.099                                          & 1.442                                                              & 1.542                  & -0.006                  & 0.973                       \\
8.1                                      & 8.075                                           & 1.618                                                              & -8.019                                          & 1.618                                                              & 1.986                  & 0.028                   & 0.961                       \\
9.1                                      & 8.936                                           & 1.811                                                              & -9.197                                          & 1.828                                                              & 2.586                  & -0.130                 & 0.957                       \\
10.1                                     & 10.078                                          & 2.023                                                              & -10.055                                         & 2.026                                                              & 2.730                  & 0.011                   & 0.971                       \\ \bottomrule
\end{tabular}%
%}
\end{table}

==> Tables/Old/main_scenario1_20.tex <==
\begin{table}[H]
\centering
\scriptsize
\caption{Simulations' results for the first scenario (20 clusters)}
\label{tab:20clusters}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc}
\multicolumn{1}{l}{}                     & \multicolumn{7}{c}{\textit{Treatment Effects}}                                                                                                                                                                                                  \\ \cline{2-8} 
\multicolumn{1}{l}{\textit{Effect Size}} & 
$\hat{\tau}_{\ell_1}$ &$\hat{se}(\hat{\tau}_{\ell_1})$ & 
$\hat{\tau}_{\ell_2}$ & $\hat{se}(\hat{\tau}_{\ell_2})$ & MSE                     & Bias                     & Coverage  \\ \hline
0.1                                      & 0.053                       & 0.286                                          & -0.072                      & 0.284                                          & 0.061                   & -0.010                   & 0.929                        \\
1.1                                      & 1.120                       & 0.382                                          & -1.102                      & 0.377                                          & 0.145                   & 0.009                    & 0.954                        \\
2.1                                      & 2.102                       & 0.538                                          & -2.114                      & 0.538                                          & 0.270                   & -0.006                   & 0.949                        \\
3.1                                      & 3.105                       & 0.710                                          & -3.140                      & 0.721                                          & 0.468                   & -0.018                   & 0.946                        \\
4.1                                      & 4.055                       & 0.905                                          & -4.198                      & 0.947                                          & 0.848                   & -0.072                   & 0.948                        \\
5.1                                      & 5.058                       & 1.100                                          & -5.034                      & 1.108                                          & 1.132                   & 0.012                    & 0.940                        \\
6.1                                      & 6.155                       & 1.332                                          & -6.034                      & 1.306                                          & 1.609                   & 0.061                    & 0.933                        \\
7.1                                      & 7.058                       & 1.519                                          & -7.036                      & 1.521                                          & 2.000                   & 0.011                    & 0.954                        \\
8.1                                      & 8.141                       & 1.737                                          & -8.118                      & 1.755                                          & 2.919                   & 0.011                    & 0.961                        \\
9.1                                      & 9.130                       & 1.952                                          & -9.160                      & 1.949                                          & 3.313                   & -0.015                   & 0.959                        \\
10.1                                     & 10.088                      & 2.150                                          & -10.071                     & 2.142                                          & 4.021                   & 0.008                    & 0.947                        \\ \midrule
\multicolumn{1}{l}{}                     & \multicolumn{7}{c}{\textit{Spillover Effects}}                                                                                                      \\ \cline{2-8} 
\multicolumn{1}{l}{}          & 
$\hat{\delta}_{\ell_1}$ & $\hat{se}(\hat{\delta}_{\ell_1})$ & 
$\hat{\delta}_{\ell_2}$ & $\hat{se}(\hat{\delta}_{\ell_2})$ & {MSE} & {Bias} & {Coverage} \\ \hline           
0.1                                      & 0.085                       & 0.234                                          & -0.139                      & 0.255                                          & 0.064                   & -0.027                   & 0.929                        \\
1.1                                      & 1.092                       & 0.300                                          & -1.106                      & 0.297                                          & 0.075                   & -0.007                   & 0.967                        \\
2.1                                      & 2.072                       & 0.393                                          & -2.083                      & 0.396                                          & 0.132                   & -0.006                   & 0.965                        \\
3.1                                      & 3.067                       & 0.509                                          & -3.084                      & 0.511                                          & 0.208                   & -0.009                   & 0.973                        \\
4.1                                      & 4.124                       & 0.641                                          & -4.088                      & 0.639                                          & 0.296                   & 0.018                    & 0.971                        \\
5.1                                      & 5.118                       & 0.772                                          & -5.052                      & 0.772                                          & 0.436                   & 0.033                    & 0.974                        \\
6.1                                      & 6.082                       & 0.900                                          & -6.154                      & 0.915                                          & 0.611                   & -0.036                   & 0.972                        \\
7.1                                      & 7.114                       & 1.042                                          & -7.101                      & 1.040                                          & 0.802                   & 0.007                    & 0.968                        \\
8.1                                      & 8.023                       & 1.183                                          & -8.156                      & 1.185                                          & 1.027                   & -0.067                   & 0.975                        \\
9.1                                      & 9.106                       & 1.312                                          & -9.139                      & 1.323                                          & 1.262                   & -0.017                   & 0.979                        \\
10.1                                     & 10.210                      & 1.465                                          & -10.151                     & 1.460                                          & 1.472                   & 0.029                    & 0.976                        \\ \bottomrule \\
\end{tabular}%
%}
\end{table}

==> Tables/Old/main_scenario1_30.tex <==


\begin{table}[H]
\centering
\scriptsize
\caption{Simulations' results for the first scenario (30 clusters)}
\label{tab:30clusters}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc}
\multicolumn{1}{l}{} & \multicolumn{7}{c}{\textit{Treatment Effects}}                                                                                             \\ \cline{2-8} 
\textit{Effect Size} & $\hat{\tau}_{\ell_1}$ & $\hat{se}(\hat{\tau}_{\ell_1})$ & $\hat{\tau}_{\ell_2}$ & $\hat{se}(\hat{\tau}_{\ell_2})$ & MSE   & Bias   & Coverage \\ \hline
0.1                  & 0.092              & 0.238                        & -0.068             & 0.230                                 & 0.016 & 0.012  & 1.000    \\
1.1                  & 1.083              & 0.311                        & -1.115             & 0.306                                 & 0.091 & -0.016 & 0.950    \\
2.1                  & 2.101              & 0.435                        & -2.107             & 0.436                                 & 0.170 & -0.003 & 0.949    \\
3.1                  & 3.104              & 0.584                        & -3.113             & 0.588                                 & 0.305 & -0.005 & 0.953    \\
4.1                  & 4.086              & 0.754                        & -4.114             & 0.746                                 & 0.546 & -0.014 & 0.946    \\
5.1                  & 5.168              & 0.921                        & -5.170             & 0.931                                 & 0.794 & -0.001 & 0.956    \\
6.1                  & 6.110              & 1.091                        & -6.059             & 1.074                                 & 1.041 & 0.025  & 0.956    \\
7.1                  & 7.133              & 1.259                        & -7.135             & 1.251                                 & 1.422 & -0.001 & 0.960    \\
8.1                  & 8.078              & 1.420                        & -7.952             & 1.409                                 & 1.729 & 0.063  & 0.946    \\
9.1                  & 9.199              & 1.618                        & -9.047             & 1.580                                 & 2.264 & 0.076  & 0.961    \\
10.1                 & 10.148             & 1.763                        & -10.171            & 1.765                                 & 2.862 & -0.012 & 0.958    \\ \midrule
 \multicolumn{1}{l}{}                     & \multicolumn{7}{c}{\textit{Spillover Effects}}                                                                                                      \\ \cline{2-8} 
\multicolumn{1}{l}{}
                     & $\hat{\delta}_{\ell_1}$ & $\hat{se}(\hat{\delta}_{\ell_1})$ & $\hat{\delta}_{\ell_2}$ & $\hat{se}(\hat{\delta}_{\ell_2})$          & MSE   & Bias   & Coverage \\ \hline
0.1                  & 0.022              & 0.208                        & -0.086             & 0.213                        & 0.019 & -0.032 & 0.967    \\
1.1                  & 1.082              & 0.249                        & -1.108             & 0.244                        & 0.056 & -0.013 & 0.964    \\
2.1                  & 2.080              & 0.322                        & -2.115             & 0.326                        & 0.083 & -0.017 & 0.974    \\
3.1                  & 3.094              & 0.423                        & -3.065             & 0.418                        & 0.132 & 0.015  & 0.969    \\
4.1                  & 4.119              & 0.528                        & -4.083             & 0.525                        & 0.209 & 0.018  & 0.973    \\
5.1                  & 5.092              & 0.634                        & -5.110             & 0.637                        & 0.263 & -0.009 & 0.983    \\
6.1                  & 6.085              & 0.745                        & -6.126             & 0.746                        & 0.384 & -0.020 & 0.975    \\
7.1                  & 7.061              & 0.857                        & -7.160             & 0.860                        & 0.517 & -0.050 & 0.977    \\
8.1                  & 8.101              & 0.974                        & -8.051             & 0.973                        & 0.695 & 0.025  & 0.979    \\
9.1                  & 9.111              & 1.088                        & -9.103             & 1.091                        & 0.827 & 0.004  & 0.984    \\
10.1                 & 10.184             & 1.215                        & -10.123            & 1.201                        & 0.993 & 0.030  & 0.981 
 \\ \bottomrule
\end{tabular}%
%}
\end{table}

==> Tables/Old/main_scenario2.tex <==
\begin{table}[H]
\centering
\scriptsize
\caption{Simulations' results for second scenario (30 clusters)}
\label{tab:second_scenario}
%\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccc}
\multicolumn{1}{l}{} & \multicolumn{7}{c}{\textit{Treatment Effects}}                                                                                     \\ \cline{2-8} 
\textit{Effect Size} & $\hat{\tau}_{\ell_{\tau1}}$ & $\hat{se}(\hat{\tau}_{\ell_{\tau1}})$ & $\hat{\tau}_{\ell_{\tau2}}$ & $\hat{se}(\hat{\tau}_{\ell_{\tau2}})$ & MSE    & Bias   & Coverage \\ \hline
0.1                  & 0.194              & 0.254                        & 0.351              & 0.241                        & 0.059  & 0.072  & 0.964    \\
1.1                  & 1.103              & 0.310                        & 3.239              & 0.607                        & 0.223  & -0.029 & 0.942    \\
2.1                  & 2.088              & 0.438                        & 6.379              & 1.121                        & 0.650  & 0.034  & 0.952    \\
3.1                  & 3.100              & 0.589                        & 9.317              & 1.634                        & 1.226  & 0.008  & 0.970    \\
4.1                  & 4.113              & 0.756                        & 12.285             & 2.137                        & 2.353  & -0.001 & 0.945    \\
5.1                  & 5.120              & 0.917                        & 15.418             & 2.708                        & 4.106  & 0.069  & 0.944    \\
6.1                  & 6.106              & 1.074                        & 18.263             & 3.159                        & 5.469  & -0.015 & 0.947    \\
7.1                  & 7.086              & 1.241                        & 21.312             & 3.712                        & 6.246  & -0.001 & 0.955    \\
8.1                  & 8.167              & 1.433                        & 24.257             & 4.209                        & 8.790  & 0.012  & 0.949    \\
9.1                  & 9.028              & 1.569                        & 27.099             & 4.671                        & 9.975  & -0.136 & 0.954    \\
10.1                 & 10.024             & 1.733                        & 30.617             & 5.288                        & 14.454 & 0.120  & 0.951    \\ \hline
                     & \multicolumn{7}{c}{\textit{Spillover Effects}}                                                                                     \\ \cline{2-8} 
                     & $\hat{\delta}_{\ell_{\delta1}}$ & $\hat{se}(\hat{\delta}_{\ell_{\delta1}})$ & $\hat{\delta}_{\ell_{\delta2}}$ & $\hat{se}(\hat{\delta}_{\ell_{\delta2}})$ & MSE    & Bias   & Coverage \\ \hline
0.1                  & 0.086              & 0.187                        & 0.281              & 0.209                        & 0.041  & -0.017 & 1.000    \\
1.1                  & 1.089              & 0.248                        & 3.321              & 0.444                        & 0.105  & 0.005  & 0.968    \\
2.1                  & 2.116              & 0.326                        & 6.325              & 0.773                        & 0.237  & 0.021  & 0.977    \\
3.1                  & 3.120              & 0.421                        & 9.313              & 1.114                        & 0.491  & 0.016  & 0.980    \\
4.1                  & 4.109              & 0.527                        & 12.277             & 1.455                        & 0.832  & -0.007 & 0.972    \\
5.1                  & 5.123              & 0.637                        & 15.407             & 1.816                        & 1.441  & 0.065  & 0.976    \\
6.1                  & 6.119              & 0.746                        & 18.341             & 2.159                        & 1.990  & 0.030  & 0.972    \\
7.1                  & 7.074              & 0.858                        & 21.393             & 2.516                        & 2.177  & 0.033  & 0.979    \\
8.1                  & 8.095              & 0.976                        & 24.312             & 2.854                        & 3.168  & 0.003  & 0.974    \\
9.1                  & 9.048              & 1.090                        & 27.264             & 3.210                        & 3.953  & -0.044 & 0.975    \\
10.1                 & 10.053             & 1.201                        & 30.416             & 3.565                        & 4.610  & 0.034  & 0.980    \\ \hline
\end{tabular}%
%}
\end{table}

==> Tables/smoothed.tex <==
% smoothed_two_main_spillover_effects_composite_3000

\begin{table}[H]
\scriptsize
\centering

\begin{tabular}{cccccccc}
\multicolumn{1}{l}{}                  & \multicolumn{7}{c}{Treatment Effects}                                                                                                                 \\ \cline{2-8} 
\multicolumn{1}{l}{Effect Size}       & $\hat{\tau}_{\ell_1}$   & $\hat{se}(\hat{\tau}_{\ell_1})$   & $\hat{\tau}_{\ell_2}$   & $\hat{se}(\hat{\tau}_{\ell_2})$   & MSE   & Bias   & Coverage \\ \hline
0                                     & 0.118                   & 0.188                             & -0.216                  & 0.171                             & 0.043 & 0.161  & 0.913    \\
\rowcolor{gray!10} 1 & 1.055                   & 0.236                             & -1.025                  & 0.219                             & 0.051 & 0.040  & 0.956    \\
2                                     & 2.007                   & 0.306                             & -2.017                  & 0.311                             & 0.089 & 0.012  & 0.955    \\
\rowcolor{gray!10} 3 & 3.012                   & 0.423                             & -3.003                  & 0.415                             & 0.175 & 0.007  & 0.963    \\
4                                     & 4.012                   & 0.530                             & -3.956                  & 0.522                             & 0.266 & -0.016 & 0.949    \\
\rowcolor{gray!10} 5 & 4.964                   & 0.643                             & -4.991                  & 0.644                             & 0.385 & -0.023 & 0.941    \\
6                                     & 6.022                   & 0.768                             & -5.985                  & 0.765                             & 0.554 & 0.003  & 0.951    \\
\rowcolor{gray!10} 7 & 7.027                   & 0.886                             & -7.025                  & 0.887                             & 0.715 & 0.026  & 0.960    \\
8                                     & 8.045                   & 1.006                             & -8.015                  & 1.007                             & 0.952 & 0.030  & 0.958    \\
\rowcolor{gray!10} 9 & 9.018                   & 1.131                             & -9.000                  & 1.117                             & 1.087 & 0.009  & 0.954    \\
10                                    & 9.946                   & 1.233                             & -9.970                  & 1.230                             & 1.314 & -0.042 & 0.954    \\ \hline
\multicolumn{1}{l}{}                  & \multicolumn{7}{c}{Spillover Effects}                                                                                                                 \\ \cline{2-8} 
\multicolumn{1}{l}{}                  & $\hat{\delta}_{\ell_1}$ & $\hat{se}(\hat{\delta}_{\ell_1})$ & $\hat{\delta}_{\ell_2}$ & $\hat{se}(\hat{\delta}_{\ell_2})$ & MSE   & Bias   & Coverage \\ \hline
0                                     & 0.128                   & 0.162                             & -0.147                  & 0.158                             & 0.029 & 0.141  & 1.000    \\
\rowcolor{gray!10} 1 & 1.026                   & 0.181                             & -1.013                  & 0.176                             & 0.030 & 0.020  & 0.965    \\
2                                     & 2.004                   & 0.229                             & -2.011                  & 0.231                             & 0.039 & 0.007  & 0.976    \\
\rowcolor{gray!10} 3 & 2.985                   & 0.295                             & -2.981                  & 0.296                             & 0.072 & -0.017 & 0.970    \\
4                                     & 4.003                   & 0.370                             & -3.965                  & 0.370                             & 0.099 & -0.016 & 0.978    \\
\rowcolor{gray!10} 5 & 4.997                   & 0.448                             & -5.006                  & 0.449                             & 0.143 & 0.002  & 0.981    \\
6                                     & 5.999                   & 0.530                             & -5.997                  & 0.529                             & 0.204 & -0.002 & 0.976    \\
\rowcolor{gray!10}7  & 6.976                   & 0.607                             & -7.006                  & 0.608                             & 0.254 & -0.009 & 0.985    \\
8                                     & 8.009                   & 0.689                             & -7.993                  & 0.688                             & 0.343 & 0.001  & 0.977    \\
\rowcolor{gray!10} 9 & 9.000                   & 0.771                             & -8.958                  & 0.769                             & 0.395 & -0.021 & 0.981    \\
10                                    & 10.026                  & 0.855                             & -9.995                  & 0.854                             & 0.483 & 0.011  & 0.985    \\ \hline
\end{tabular}

\caption{Simulations' results for the first scenario with smoothed response.}
\label{tab:smoothed}
\end{table}
